Is ChatGPT the Ultimate Programming Assistant -- How far is it?

Recently, the ChatGPT LLM has received great attention: it can be used as a bot for discussing source code, prompting it to suggest changes, provide descriptions or even generate code. Typical demonstrations generally focus on existing benchmarks, which may have been used in model training (i.e., data leakage). To assess the feasibility of using an LLM as a useful assistant bot for programmers, we must assess its realistic capabilities on unseen problems as well as its capabilities on various tasks. In this paper, we present an empirical study of ChatGPT's potential as a fully automated programming assistant, focusing on the tasks of code generation, program repair, and code summariziation. The study investigates ChatGPT's performance on common programming problems and compares it with state-of-the-art approaches on two benchmarks. Among several findings, our study shows that ChatGPT is effective in dealing with common programming problems. However, our experiments also reveal limitations in terms of its attention span: detailed descriptions will constrain the focus of ChatGPT and prevent it from leveraging its vast knowledge to solve the actual problem. Surprisingly, we have identified the ability of ChatGPT to reason the original intention of the code. We expect future work to build on this insight for dealing with the open question of the oracle problem. Our findings contribute interesting insights to the development of LLMs for programming assistance, notably by demonstrating the importance of prompt engineering, and providing a better understanding of ChatGPT's practical applications for software engineering.

==> 7.availability.tex <==
\section{Availability}
\label{sec:availability}

All the artefacts of this study are available in the following public repository:
\begin{center}
	\url{https://}
\end{center}

==> exp3_legacy.tex <==
\subsection{ChatGPT for Code Summarization}
\label{subsec:rq3}

\noindent
{\bf [Experiment Goal]:} We aim to explore the ability of ChatGPT on code explanation. To do so, we evaluate whether ChatGPT can explain the intention of correct and incorrect codes against the description of programming problems.

\noindent
{\bf [Experiment Design]:} 
Given a programming problem, correct codes tend to 
achieve the same goal by implementing intended behaviors to satisfy associated specifications. In other words, all the correct codes exhibit semantically the same intention. On the contrary, the incorrect codes fail to test suites, meaning they carry semantically different intentions. Therefore, we consider evaluating whether the ChatGPT-generated intentions for correct and incorrect codes are significantly different. First, we request ChatGPT to explain the intention (natural language) of 2443 correct codes and 1783 incorrect codes in Refactory respectively (see the prompt in Section~\ref{chatgpt_application}). Second, we leverage Bert~\cite{devlin2018bert}, a widely used pre-trained large language model, to produce the semantic embedding representations of the above intentions of the codes and the problem descriptions. Finally, we devise two experiments to explore the cosine similarity distributions between ChatGPT-generated intentions (based on embeddings) for correct and incorrect codes as follows:
\begin{enumerate}[leftmargin=*]
\item {\bf Experiment 1}: We aim to investigate how ChatGPT performs in retrieving code intention for incorrect and correct code. 
We compute the distribution of similarities between intentions generated for correct code and the ground-truth problem descriptions, which we compare against the distribution of similarities between intentions generated for incorrect code and the ground-truth problem descriptions. If ChatGPT is accurate in describing the intention of code, then these two distributions should be significantly different: correct code intention should be closer to the ground truth description, while incorrect code intention should farther.
\item {\bf Experiment 2}: We aim to investigate the pairwise similarity distribution of the generated intentions for all correct code samples, in comparison to the similarity distribution of the generated intentions for all incorrect code samples.
These two distributions should be significantly different because all correct code samples should carry the same intention while incorrect code samples should have diverse intentions.%\scc{Cannot follow.}\tian{rephrased}
\end{enumerate}


\noindent
{\bf [Experimental Results]:} 
Figure~\ref{fig:distribution1} shows the result of {\bf Experiment 1}. The similarity distribution between the intent of incorrect code and the problem description is not significantly different from the similarity between correct code and the problem description.
Likewise, in Figure~\ref{fig:distribution2} ({\bf Experiment 2}), we also find no significant difference between the two similarity distributions.
However, the only exception is the distribution in the second problem.

\begin{figure}[h]
	\includegraphics[width=1\columnwidth]{fig/distribution1.pdf}
	\vspace{-3mm}
	\caption{Similarity distribution between intentions of correct codes and problem description {\em vs} similarity distribution between intentions of incorrect codes and problem description.}
	\label{fig:distribution1}
\end{figure}

% \vspace{-3mm}

\begin{figure}[h]
	\includegraphics[width=1\columnwidth]{fig/distribution2.pdf}
	\vspace{-3mm}
	\caption{Similarity distribution between intentions of correct codes {\em vs} similarity distribution between intentions of incorrect codes.}
	\label{fig:distribution2}
\end{figure}
% \todo{MWW}
Based on the observation, we further explore the characteristics of correct and incorrect codes in different problems that allow ChatGPT to whether successfully distinguish their intentions. As we mentioned, the second problem requires three functions to be implemented. 
% Our intuition is that ChatGPT is more capable of code explanation if more functions are given. 
To investigate the effect of the multi-functions, we separate the three single functions from the codes in the second problem to reproduce the experiments. We found the intentions of (in)correct can be distinguished by ChatGPT for functions `unique\_month' and `contain\_unique\_days' while not for `unique\_day'. After manual inspection, we find that many of the incorrect implementations of functions `unique\_month' and `contain\_unique\_days' only contain a single return statement without other code tokens (an example in Figure~\ref{fig:wrong_2_213}), meaning they have an obvious different intention that thus can be distinguished.
On the contrary, as for the other problems, ChatGPT is not able to identify the intention of incorrect implementations that need minimal changes toward the correct version. Figure~\ref{fig:307} shows such a typical example. In this example, the presented code is incorrect due to the lack of a return statement. However, when being asked about the intention of this code, ChatGPT explains that {\em this function {\bf returns} a new list containing only the unique elements}, even though there is no such return statement in this code. To avoid the effect of the function name, we replace the function name with `a'. We then still observe the same result. Upon my response that told ChatGPT there is no such a return statement, ChatGPT acknowledged its mistake of overlooking the absence of a return statement. Overall, the results imply that ChatGPT is not able to explain the intention of the given codes precisely and has limited attention (as implied in RQ-2). It seems to try to synthesize the most probable content based on its training corpus (there is usually a return statement).
% These results imply that ChatGPT can not identify and explain the different intentions of correct and incorrect codes for most problems except for problem 2. 

However, everything has two sides. The results exceptionally reflect that ChatGPT can reason the original intention of incorrect codes (e.g. the function should return a new list), although its explanation about the current codes may be wrong. 
This finding enables ChatGPT to address the oracle problem: in test generation, we do not always have a precise specification of what the output should be. Given a correctness-unknown code snippet without the test suites, ChatGPT can help reason the original intention of the code for programmers. With this intention, programmers can determine the expected output for a test input, and design the test case accordingly. We validate our speculation by analyzing 39 sampled incorrect codes that ChatGPT can identify the defects of 30 of them by suggesting the original intentions and automatically generating test cases.

\begin{figure}[h]
	\includegraphics[width=1\columnwidth]{fig/307.pdf}
	% \vspace{-6mm}
	\caption{The intention explanation of ChatGPT for an incorrect implementation for the problem {\em Duplicate Elimination}.}
	\label{fig:307}
\end{figure}

% \find{{\bf \ding{45} RQ-3 }$\blacktriangleright$ChatGPT is unable to provide a precise explanation of the intention of the given code, but it can identify the original intention of the code.$\blacktriangleleft$}

% \begin{lstlisting}[language=Python]
% def remove_extras(lst):
%     t=[]
%     for i in lst:
%         if i not in t:
%             t.append(i)
% \end{lstlisting}

% \begin{figure}[!t]
%     \centering
%     \scriptsize
%     \lstinputlisting[language=Python,linewidth={\linewidth},frame=tb,basicstyle=\ttfamily,basicstyle=\footnotesize ]{listings/307.list}
%     \caption{307-th incorrect code for problem Duplicate
% Elimination.}
%     \label{fig:307}
% \end{figure}

